Expand-and-Quantize: Unsupervised Semantic Segmentation Using High-Dimensional Space and Product Quantization

Unsupervised semantic segmentation (USS) aims to discover and recognize meaningful categories without any labels. For a successful USS, two key abilities are required: 1) information compression and 2) clustering capability. Previous methods have relied on feature dimension reduction for information compression, however, this approach may hinder the process of clustering. In this paper, we propose a novel USS framework called Expand-and-Quantize Unsupervised Semantic Segmentation (EQUSS), which combines the benefits of high-dimensional spaces for better clustering and product quantization for effective information compression. Our extensive experiments demonstrate that EQUSS achieves state-of-the-art results on three standard benchmarks. In addition, we analyze the entropy of USS features, which is the first step towards understanding USS from the perspective of information theory.

==> table/module.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{1pt}
\vspace{-0.25cm}
\begin{subtable}[h]{0.29\textwidth}
\centering
    % \captionsetup{font=small}
    \vspace{-0.35cm}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    Model & CocoStuff-27 & Potsdam & Cityscapes  \\
        \midrule
        STEGO & 0.020 & 0.021 & 0.020 \\
        \textbf{EQUSS} & 0.020 & 0.024 & 0.026 \\
        \bottomrule
    \end{tabular}
    }
    % \caption{
    % }
    \vspace{-0.35cm}
    % \vspace{-0.45cm}
	\end{subtable}
	\hfill
    \begin{subtable}[h]{0.165\textwidth}
    \centering
    % \captionsetup{font=small}
    % \vspace{-0.35cm}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    Method & mIoU & Acc. \\ % & L.mIoU & L.Acc. \\
        \midrule
        HP(ViT-S)$\dagger$ & 16.04 & 73.08 \\ % & 82.4 & 00.0\\
        \textbf{+Ours} & \textbf{17.42} & \textbf{78.91} \\ % & TODO & TODO \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{-0.45cm}
    % \caption{
    % }
    % \vspace{-0.35cm}
    \end{subtable}
    \centering
    \vspace{-0.2cm}
    \caption{\small{(left) $L_{corr}$ computation time (sec) averaged over 25 runs. 
    (right) Performance on Cityscapes.
    $\dagger$ indicates our reproduced results.
    % (right) Effect of our module integrated into another method.
    % U:Unsupervised, L:Linear.
    The results are without CRF post-processing.}
    }
    % }
    \vspace{-0.35cm}
    \label{tab:speed_module}
\end{table}


==> table/quantize.tex <==
\setlength{\tabcolsep}{9pt}
\begin{table}[t]
    \centering
    \captionsetup{font=small}
    % \vspace{-0.35cm}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{Quant. method} & \multicolumn{2}{c}{CocoStuff-27} & \multicolumn{2}{c}{Cityscapes}  &
    Potsdam\\
    & mIoU & Acc. &  mIoU & Acc. &  Acc. \\
        \midrule
        Soft relaxation & 22.48 & 46.96  & 20.55 & 73.3 &  61.57 \\
        Gumbel softmax &  25.29 & 52.26 & 21.34 & 76.9  &  81.61\\ 
        % Gumbel\_none & 48.1 & 13.8 & 54.2 & 13.9 & 1 & 1\\ 
        \textbf{Ours (Eq. (3,4))} & \textbf{25.8}  & \textbf{53.8} & \textbf{22.0} & \textbf{79.9}  & \textbf{82.0}\\ 
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.3cm}
    \caption{Comparison of quantization methods.
    }
    \vspace{-0.7cm}
    \label{tab:quantization}
\end{table}
\setlength{\tabcolsep}{6pt}
